Inverse homogenization problem for the Drichlet problem for Poisson equation for $W^{-1,\infty}$ potential

We consider Poisson problems $-\Delta u^\varepsilon=f$ on perforated domains, and characterize the limit of $u^\varepsilon$ as the solution to $(-\Delta+\mu)u=f$ on domain $\Omega\subset\mathbb{R}^d$ with some potential $\mu\in W^{-1,\infty}(\Omega).$ It is known that $\mu$ is related to the capacity of holes when $\mu\in L^\infty(\Omega).$ In this paper, we characterize $\mu$ as the limit of the density of the capacity of holes also for many $\mu\in W^{-1,\infty}(\Omega).$ We apply the result for the inverse homogenization problem, i.e. we construct holes corresponding to the given potential $\mu\in L^d(\Omega)+L^\infty(\delta_S)$ where $\delta_S$ is a surface measure.

==> p/98figcube.tex <==
\begin{figure}\centering
\begin{overpic}[width=8cm]{p/fig/peri}
\put(45,22){$\Omega$}
%\put(48,48){$K_i^\ep$}
\end{overpic}
\caption{A domain perforated by periodic balls\label{figperi}}
\end{figure}
